Variable Record Table: A Run-time Solution for Mitigating Buffer Overflow Attack

We present a novel approach to mitigate buffer overflow attack using Variable Record Table (VRT). Dedicated memory space is used to automatically record base and bound information of variables extracted during runtime. We instrument frame pointer and function(s) related registers to decode variable memory space in stack and heap. We have modified Simplescalar/PISA simulator to extract variables space of six (6) benchmark suites from MiBench. We have tested 290 small C programs (MIT corpus suite) having 22 different buffer overflow vulnerabilities in stack and heap. Experimental results show that our approach can detect buffer overflow attack with zero instruction overhead with the memory space requirement up to 13Kb to maintain VRT for a program with 324 variables.

==> future.tex <==
\section{Future Research}

In this work, we assume compiler to provide the bound information beforehand for the register(variable). Finding base and bound information of variables from the object file will make the hardware to stand alone to detect the unauthorized access of the array element. Further pointer and its operation can also be studied to broaden the scope of this architecture.  

==> reviewer_comment_full.tex <==
****************************************
Reviewer #1 Comments
****************************************
The paper has some grammatical mistakes that made it harder for me to read for the firs time. 
(Addressed)

The VRT concept seems promising to detect buffer overflow . However, I wonder how the VRT can handle programs with large number of variables and data structures. The authors discuss some results on MiBench suites and MIT Corpus suite. They do not discuss standard benchmarks such SPEC CPU2017 (integer and floating point). I believe the larger the number of variables and data structures, the larger the VRT has to be. Therefore, what is the limit that the VRT can handle? Would the VRT become too large to be realistically implemented? Would a large VRT impose latency and power overhead on the CPU? The authors need to clearly address these questions! 

-- Fig 7 from trans paper

I would suggest more pictorial illustration of the VRT table on detecting buffer overflow.

Finally, I think the paragraph on page 2 in the right column (lower right corner) has some mistakes referencing Figure 4.

-- 

****************************************
Reviewer #2 Comments
****************************************
The paper proposes an approach to detect out-of-bound access to objects in a program. The approach relies on a base and bound table information (VRT) that is filled during program runtime. Out-of-bond memory access is not a new problem but is still relevant.

The overall idea seems to have merit, however, the text needs much improvement. The first three pages of the paper are almost entirely dedicated to background and preliminaries. Half of page 3 (section III-C and on) are dedicated to explaining the approach and discussing results. That should be the large of the paper. For instance, instead of explaining the semantics of malloc, realloca and free, expand on shadow stack and how you use it. How do you store "meta-data of variables in a transparent manner" ?
I don't really understand what you are trying to convey with figure 5. Do you have 3 different tables in memory? (Stack, traditional shadow stack and VRT?) Are you storing the same return address R0 in both Stack and traditional shadow stack? How does that relate to object base/bound?

For the VRT, how do you know to which variable each entry is associated with? Do you have to do a table walk to figure this out? Or do you keep an extra pointer in the stack?

Please improve the description of the associated bit. What do you mean by "differentiate entries of a function with other"? You can only differentiate between two functions? What happens if the program has 3 functions?

You propose using 8 bits for bound. What happens if I have an array with 1K entries? What about 1M entries? (that is a small program for me).

Please give a brief overview of the micro-architecture in [13]. What is the ISA? Is it in-order? OoO? How many stages? etc...

I don't understand the "Unchecked variable index" section. Yes, that is an out-of-bound access, so what? How does your framework solves the issue?

In your results, you need to report memory overhead as a percentage of program memory. For instance, CRC32 has 9 variables, I will assume they are all 64 bits. For each variable you are adding 41 bits, this is a 64\% overhead. For arrays, your overhead will be smaller, but then again, the 8 bits allocated to bound are not sufficient to cover large arrays, so the minimum overhead you will have is for a 256 entry array of 64 bit entries (~0.3\%). 0.3\% is not unacceptable, but you cannot sell that as a flat 13KB. 

In the abstract you claim that you do not add instruction to the program, I cannot verify that claim since there is not a lot of explanation about how the approach works. This needs to be clear.

You mentioned other works that try to solve the same problem. How does your approach compare?

The abstract could be improved. Give more context to the work being done. Start with a statement of why the problem you are trying to solve is important and clearly state what the problem is. Also, mention whether the table is dynamically stored in memory or in dedicated hardware.

Figure 2 is way too busy. There's just too much going on that someone unfamiliar with the topic would not be able to understand the figure (and someone familiar with the topic doesn't really need the explanation). I would suggest stacking b and c, and having the pointers go through the sides. In general, try to cross less arrows. Try to develop a bit on the caption. What is the point you are trying to make here? I would consider reducing this a lot. This is a 4 page paper and you are spending half a page with what is basically intro level programming.

You're missing a citation for MiBench. 

Minors/Typos

- Abstract "run-time ." (there is an extra space before the period)

- First paragraph: thrice

- SimpleScalar toolset[11] (missing space)

- variables access go par (?)

- "shows a depiction" -> depicts

- Make sure your negative vspaces are not causing text overlaps (page 3)

****************************************
Reviewer #3 Comments
****************************************
This paper proposes a novel approach called variable record table without instruction overhead for buffer overflow attack. The authors give the detail example to introduce the buffer overflow and the proposal. There are many grammatical errors and formatting errors in the paper. The quality of the paper should be improved. 
In Section III, the authors use lot of space in the paper to introduce static/dynamic variable space. However, the novelty is in subsection III-C, D, which is not clear. Two cases of illegal accesses are provided to explain the VRT. How about other overflow cases?
Experimental results are provided to verify the proposal. As it can be seen in Table III, attack can be successfully detected. Clarifying more details about experiment is helpful for reader to understand the success of the VRT on overflow attack.

****************************************
Reviewer #4 Comments
****************************************
This paper describes a scheme to extract base and bound information of variable space from object file during run-time.  The stored information in a table is  called Variable Record Table (VRT).

1.　I think the comparison with other works make readers understand the proposed technique clearly.

2.　13KB use for VRT in memory space is small enough? 

3.　The line 2 in column 2 in p. 3 is disturbed.

4.　In reference [14], there is no stipulation of a source.

****************************************
Reviewer #5 Comments
****************************************
No comments provided.
